A Novel Approach to Industrial Defect Generation through Blended Latent Diffusion Model with Online Adaptation

Effectively addressing the challenge of industrial Anomaly Detection (AD) necessitates an ample supply of defective samples, a constraint often hindered by their scarcity in industrial contexts. This paper introduces a novel algorithm designed to augment defective samples, thereby enhancing AD performance. The proposed method tailors the blended latent diffusion model for defect sample generation, employing a diffusion model to generate defective samples in the latent space. A feature editing process, controlled by a ``trimap" mask and text prompts, refines the generated samples. The image generation inference process is structured into three stages: a free diffusion stage, an editing diffusion stage, and an online decoder adaptation stage. This sophisticated inference strategy yields high-quality synthetic defective samples with diverse pattern variations, leading to significantly improved AD accuracies based on the augmented training set. Specifically, on the widely recognized MVTec AD dataset, the proposed method elevates the state-of-the-art (SOTA) performance of AD with augmented data by 1.5%, 1.9%, and 3.1% for AD metrics AP, IAP, and IAP90, respectively. The implementation code of this work can be found at the GitHub repository https://github.com/GrandpaXun242/AdaBLDM.git

==> main_algorithm.tex <==

\begin{algorithm}[htbp]
    \caption{Inference pseudo-code of CPR}  
    \label{alg:infer}
    \LinesNumbered  
    \KwIn{Two pre-trained feature extractors of DenseNet$201$: $\Psi_{D}^l(\cdot), l \in
    \{1, 2\}$; GRB $\Psi_{G}(\cdot)$, global feature oracle $\mathcal{G}_{\text{ref}}$;
    LRB $\Psi_{L}(\cdot)$; local feature oracles with multi-scale
    $\mathcal{L}^l_{\text{ref}}, l \in \{1, 2\}$; FEB $\Psi_{F}(\cdot)$; foreground
    estimation map set $\mathcal{F}_{\text{ref}}$; number of nearest neighbors $K$; test
    image $\II_{\text{tst}}$.
    }  
    \KwOut{Anomaly score map $\text{A}_{\text{tst}}$ and anomaly score $\alpha_{\text{tst}}$ for $\II_{\text{tst}}$.}  % 输出
    \textbf{Algorithm:}\\
    \tcc{{Feature extraction}}
    \For{$l \in \{1, 2\}$}{
        $\mathfrak{P}_{\text{tst}}^l = \Psi_{D}^l(\II_{\text{tst}})$
    }
    $\mathfrak{G}_{\text{tst}}, \text{F}_{\text{tst}} =
    \Psi_{G}(\mathfrak{P}_{\text{tst}}^1),\Psi_{F}(\mathfrak{P}_{\text{tst}}^1)$ \\
    \tcc{{Find the $K$-NNs of $\mathfrak{G}_{\text{tst}}$ in
    $\mathcal{G}_{\text{ref}}$}}
    $\boldsymbol{\beta}_{\text{knn}} = \texttt{KNN-Idx}(\mathfrak{G}_{\text{tst}},
    \mathcal{G}_{\text{ref}}) \in \mathbb{N}^{K}$\\

    $\mathcal{F}_{\text{knn}} = \mathcal{F}_{\text{ref}}[\boldsymbol{\beta}_{\text{knn}}]$\\

    $\text{F}^* = \texttt{MaxPool}(\mathcal{F}_{\text{knn}} \cup \text{F}_{\text{tst}})$ \\
    \tcc{{multiscale local retrieval}}
    $\text{A}_{\text{mul}} = \text{0} \in \mathbb{R}^{H_L \times W_L}$\\


    \For{$l \in \{1, 2\}$}
    {

        $\mathfrak{L}^l_{\text{tst}} = \Psi_{L}(\mathfrak{P}^l_{\text{tst}})$ \\

        $\mathfrak{L}^l_{\text{tst}}
        \xrightarrow{\texttt{flatten}} \mathcal{L}_{\text{tst}} = \{\vv{l}^{r, c}_{\text{tst}} \in \hanxiR^{C_L}
        \mid \forall r, c\}$ \\

        $\mathcal{L}^l_{\text{ref}}[\boldsymbol{\beta}_{\text{knn}}]
        \xrightarrow{\texttt{flatten}} \mathcal{L}_{\text{knn}} = \{\vv{l}^{r, c, j}_{\text{knn}} \in \hanxiR^{C_L}
        \mid \forall r, c, j\}$ \\
      
        \For{$r \in \{1, \dots, H_L\}$ and $c \in \{1, \dots, W_L\}$}
        {
          $\vv{l}^{\ast}_{r, c} = \texttt{LocalNN}(\vv{l}^{r, c}_{\text{tst}},
          \mathcal{L}_{\text{knn}})$ as \ref{equ:loal_retrieval}
          $\text{A}_{\text{ori}}^l[r,c] = 1 -
          \Psi_{\text{cos}}(\vv{l}^{r, c}_{\text{tst}}, \vv{l}^{\ast}_{r, c})$\\

        }
        $\text{A}_{\text{mul}} = \text{A}_{\text{mul}} +
        \texttt{UpInterp}(\text{A}_{\text{ori}}^l)$\\
    }
    \tcc{{foreground filter}}
    $\text{A}^{\ast} = \text{A}_{\text{mul}} \odot \text{F}^{\ast}$\\
    \tcc{{image-level anomaly score}}
    $\alpha^{\ast} =
    \sum_{i=1}^{T}\texttt{sort}^{\Downarrow}(\texttt{flatten}(\text{A}^{\ast}))$
\end{algorithm}



